On the equivalence between quantum and random walks on finite graphs

Quantum walks on graphs are ubiquitous in quantum computing finding a myriad of applications. Likewise, random walks on graphs are a fundamental building block for a large number of algorithms with diverse applications. While the relationship between quantum and random walks has been recently discussed in specific scenarios, this work establishes a formal equivalence between the processes on arbitrary finite graphs and general conditions for shift and coin operators. It requires empowering random walks with time heterogeneity, where the transition probability of the walker is non-uniform and time dependent. The equivalence is obtained by equating the probability of measuring the quantum walk on a given node of the graph and the probability that the random walk is at that same node, for all nodes and time steps. The result is given by the construction procedure of a matrix sequence for the random walk that yields the exact same vertex probability distribution sequence of any given quantum walk, including the scenario with multiple interfering walkers. Interestingly, these matrices allows for a different simulation approach for quantum walks where node samples respect neighbor locality and convergence is guaranteed by the law of large numbers, enabling efficient (polynomial) sampling of quantum graph trajectories (paths). Furthermore, the complexity of constructing this sequence of matrices is discussed in the general case.

==> ensemble.tex <==
\section{Simulation of quantum walk trajectories} \label{sec:ensemble}


Theorem \ref{th:qw_locality} establishes the construction procedure of a non-homogeneous random walk equivalent to a given quantum walk. Thus, the random walk can be simulated giving rise to trajectories (paths) of G. Interestingly, the random walk is statistically equivalent with the quantum walk at each time instant $t$ and the trajectories can be interpreted as trajectories related with the quantum process. In a proper language, these trajectories resemble the Feynman description of path integrals in a discrete context. The walker probability evolution from an initial condition $\ket{\Psi(0)}$ is interfered by every possible path of $t$ steps which connects  related with all the possible paths of the 

trajectories can be sampled through the simulation of the random walk, giving rise to a different procedure of simulation for 
the simulation of this random walk can  Given a graph $G = (V,E)$, quantum walk operators $S$ and $W$ and an initial condition $\ket{\psi(0)}$, let $X_t$ be a random variable which denotes the vertex seen by a classical walker at instant $t$, with distribution $\rho(t)$. Let $\beta(k)$ be the matrix computed from $S$, $W$ and $\ket{\psi(0)}$ for instant $k$ using Theorem \ref{th:qw_locality}. Now, let $\tau = \{x_0,..., x_t\}$ to denote a sampled trajectory obtained from the random walk constructed with the matrix sequence $\{\beta(0),...,\beta(t-1)\}$. As stated before, $x$ is a graph traversal where the vertex seen at instant $t$ appears with probability following Equation \ref{eq:ens_trans}, which clearly shows a dependency between two adjacent random variables.



\begin{align}
    & P[X_{k+1} = x_k+1] = P[X_{k+1} = x_{k+1} | X_{k} = x_{k}]P[X_{k} = x_k] \label{eq:ens_trans}
\end{align}

\begin{figure}
	\centering
    \begin{minipage}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{fig/Fig2(left).png}
    \end{minipage}
    \begin{minipage}[b]{0.45\textwidth}
	    \includegraphics[width=\textwidth]{fig/Fig2(right).png}
    \end{minipage}
   	\caption{Ensembles of 20 trajectories obtained using Theorem \ref{th:qw_locality} for a Hadamard-coined(left) and Grover-coined(right) walks on a 10-by-10 2-D torus with moving shift swap operators for a localized initial state $\ket{0,0} $(left edge of the origin). Each one of the solid lines corresponds to a given trajectory and the dashed line gives its empirical average of the vertex random variable per instant.}
    \label{fig:trajectories}
\end{figure}

In addition, let $\chi = \{\tau_1, ..., \tau_M\}$ be an ensemble of trajectories obtained by $M$ repetitions of the previous sampling process, exemplified in Fig.\ref{fig:trajectories}. The law of large numbers states that, as $M$ increases, the expected fraction of visits of the walkers on vertex a $u$ at instant $t$ within $\chi$ approaches $\rho(u, t)$. To depict this behavior, an empirical analysis of the total variation distance (Equation \ref{eq:tvd}) between the ensemble empirical distribution and the quantum walk distribution is reported in Fig.\ref{fig:trajectories_tvd}. % Even though each trajectory shows a dependency among its random variables, the joint distribution within the ensemble approaches independence as the ensemble size grows.

\begin{align}
    & D(p, q) = \frac{1}{2} \sum_{v}|p(v) - q(v)| \label{eq:tvd}
\end{align}

\begin{figure}
	\centering
    \begin{minipage}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{fig/Fig1(left).png}
    \end{minipage}
    \begin{minipage}[b]{0.45\textwidth}
	    \includegraphics[width=\textwidth]{fig/Fig1(right).png}
    \end{minipage}
   	\caption{Analysis of the total variation distance between the empirical distribution obtained from trajectory sampling and the quantum walk distribution of a Grover -coined walk with moving shift on a 10-by-10 2-D torus. The left figure shows the total variation value for the distribution at each instant, with different curves representing different ensemble sizes. The right figure gives the distance value for a fixed time instant when the ensemble size grows.}
    \label{fig:trajectories_tvd}
\end{figure}

The dependency of samples within the trajectory differs from the behavior of the analogous sampling process for quantum walks. Let $Y_t$ denote a random variable which represents the measurement outcome of the vertex space of the quantum walk defined by the same $S$ and $W$ operators at instant $t$. Suppose now that a sequence of $t+1$ measurements is performed on $t + 1$ identically prepared walker systems with initial condition $\ket{\psi(0)}$, each of which was evolved into a unique instant $k$, $0 \leq k \leq t +1$, leading to an ensemble of measurements $\phi = {y_0,...,y_t}$. Since the systems are independent, the nature of measurement implies that the probability for the realizations of the random variables follows Equation \ref{eq:mes_trans}.

\begin{align}
    & P[Y_{k+1} = y_{k+1} | Y_k = y_k] = P[Y_{k+1}] \label{eq:mes_trans}
\end{align}

Again, if an ensemble of measurements $\upsilon = \{\phi_1,...,\phi_M\}$ is taken into account, the fraction of times of which the vertex $u$ appears at instant $t$ will also approaches $\rho_u(t)$ as $M$ increases. The interesting behavior here is that of ensembles of different natures, of dependent and independent samples, recovering, in the sense of the law of large numbers, the same sequence of probability distributions.

\subsection{Polynomial procedure for sampling trajectories}
